Few-shot Intent Classification and Slot Filling with Retrieved Examples

Few-shot learning arises in important practical scenarios, such as when a natural language understanding system needs to learn new semantic labels for an emerging, resource-scarce domain. In this paper, we explore retrieval-based methods for intent classification and slot filling tasks in few-shot settings. Retrieval-based methods make predictions based on labeled examples in the retrieval index that are similar to the input, and thus can adapt to new domains simply by changing the index without having to retrain the model. However, it is non-trivial to apply such methods on tasks with a complex label space like slot filling. To this end, we propose a span-level retrieval method that learns similar contextualized representations for spans with the same label via a novel batch-softmax objective. At inference time, we use the labels of the retrieved spans to construct the final structure with the highest aggregated score. Our method outperforms previous systems in various few-shot settings on the CLINC and SNIPS benchmarks.

==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/abstract.tex <==
\begin{abstract}
% Few-shot learning is an important problem in natural language understanding tasks due to scenarios such as introduction of new domains and labels. 
Few-shot learning arises in important practical scenarios, such as when a natural language understanding system needs to learn new semantic labels for an emerging, resource-scarce domain.
In this paper, we explore retrieval-based methods for intent classification and slot filling tasks in few-shot settings.
Retrieval-based methods make predictions based on labeled examples in the retrieval index that are similar to the input, and thus can adapt to new domains simply by changing the index without having to retrain the model. However, it is non-trivial to apply such methods on tasks with a complex label space like slot filling.
%due to their advantage of 1) better adaptation to new domains; and 2) not requiring model retraining with new labels. 
%However, structured prediction beyond intent classification is challenging for retrieval-based methods.
To this end, we propose a span-level retrieval method that learns similar contextualized representations for spans with the same label via a novel batch-softmax objective.
At inference time, we use the labels of the retrieved spans to construct the final structure with the highest aggregated score.
Our method outperforms previous systems in various few-shot settings on the CLINC and SNIPS benchmarks.


%In this paper, we explore few-shot slot filling and intent classification with retrieved examples. 
%Because of benefits such as minimal model retraining and explainable prediction, retrieval-based non-parametric methods have been popular. Recent methods for sequence labeling tasks model token-level embedding similarities and label dependencies independently for structured prediction. However, label dependencies are not available in a new domain.
%Instead, we propose a span-level retrieval method to learn similar representations for spans and utterances of the same label.
% In this paper, we explore retrieval-based methods for tackling the few-shot intent classification and slot filling tasks due to their advantage of 1) better explainability; and 2) might not require model retraining with new intent/schema.
%\dy{"due to their advantage of ...": the two points here are kind of justified by recent research on metric learning, but retrieval (e.g. knn) is not known to work well for few-shot, but we use batch softmax to make it work}


\end{abstract}

==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/analysis.tex <==

\section{Analysis}
%We conduct further discussion and ablation studies in this section to analyze the variations of different settings. \dy{need to add some analysis on interpretability somewhere? Because prototypical is well known to perform (almost) the best in few-shot setting, even though we showed that retrieval works, reviewers can argue that our improvement is not "significant" from the results table. Then we need to highlight the benefits of retrieval models}

\subsection{Intent Classification}

\label{ana:intent}
% Different from slot filling where we only evaluate the models without re-training on the target domain to be consistent with previous research, we also evaluate all models with fine-tuning on the target domain after pre-training on the source domain for intent classification. 
% We only evaluate the models without re-training on the target domain to be consistent with previous research. However, for intent classification, we also evaluate all models with fine-tuning on the target domain after pre-training on the source domain.
% Due to space limitation, we only show 5-shot results for d=5, l=15 in Table \ref{clinc_results}. Results for other data constructions are consistent and we present them in Appendix \ref{app:clinc_results}.
% Table \ref{clinc_results} summarizes the intent classification results on CLINC for the following setting: number of source domains $d=10$, number of intents per domain $l=10$, and with 5-shot for each intent. Results on other settings have the same patterns (See Appendix~\ref{app:clinc_results}).

% \paragraph{Varying the support set at inference data.}
% Another observation is that when comparing between full support sets (\texttt{support\_set=all}) and balanced support sets (\texttt{support\_set=few}), Retriever\_Span achieves higher accuracy on source domains (97.08\% vs. 95.44\%) while lower on target domains (62.69\% vs. 75.93\%). This is reasonable because full support sets have more source domain examples to increase confusion over target domains. However, this trade-off is encouraging because we can dramatically increase target domain accuracy without degrading source domain accuracy by much. \zy{I'm not sure if this is convincing because the relative reduction is similar.}


\paragraph{Models without re-training}
The \textit{pre-train on src domain} section in Table \ref{clinc_results} shows the results of models that are only pre-trained on the source domains but \textbf{not} fine-tuned on the target domains. Classification models such as \texttt{BERT fine-tune} cannot make predictions on target domains in this setting. 
In contrast, even without seeing any target domain examples during training, retrieval-based models can still make predictions on new domains by simply including new examples in the support sets. 
With {support\_set=all}, \texttt{Retriever} achieves 97.08\% on the source domain while \texttt{Proto} performs worse than \texttt{BERT fine-tune}, consistent with previous findings \cite{meta_dataset}.
\texttt{Retriever} achieves the best accuracy (75.93\%) on target domains with a balanced support set on all intents ({support\_set=balance}).
More importantly, \texttt{Retriever} also achieves competitive accuracy on source domains (95.44\%), demonstrating that our proposed model achieves the best of both worlds even without re-training on new domains. 
% \zy{Issue: I didn't mention minmax and Retriever\_Proto at all.} \dy{It's fine not to mention minmax and proto here. But we should talk about performance before any training (initial BERT) right? Not sure how to fit in this}

\paragraph{Varying the support set at inference time} 
%\dy{this is kind of orthogonal than the rest of the analysis. Not sure if this is the best way to present/highlight it here.}
%In each setting, we show model prediction accuracy under three support sets in the row sections in Table~\ref{clinc_results}. 
% For retrieval-based methods, the construction of the support set is critical to model performance.
The construction of the support set is critical to retrieval-based methods.
In Table~\ref{clinc_results}, we present the model performances under different support settings (all, balance, tgt).
The {support\_set=tgt} setting serves as an upper bound for the target domain accuracy for both \texttt{Retriever} and \texttt{Proto} methods.
In general, 
% our retrieval-based methods 
\texttt{Retriever}
achieve the best performance on the source domain intents when we use full support sets (support\_set=all). 
In comparison, if we use a balanced support set (support\_set=balance), we can achieve much higher accuracy on the target domain while having a slight degradation on the source domain intents prediction.
This is because full support sets have more source domain examples to increase confusion over target domains. 
%However, this trade-off is encouraging because we can dramatically increase target domain accuracy without degrading source domain accuracy by much. \zy{I'm not sure if this is convincing because the relative reduction is similar.} 


%Retriever-based models still perform well given that there are 100 classes in the source domain and 50 classes in the target domain.
%Results from the original BERT checkpoint suggest that without any training, retrieval-based models can still perform well given that there are 100 classes in the source domain and 50 classes in the target domain. If we train the model on the source domain data, the traditional BERT fine-tune model cannot map query to classes in the target domain with a linear classification model where the linear layer is pre-defined so that we can only classify utterances from the source domains. Proto\_Span does not perform well (95.73) compared to BERT fine-tune on the source domain (96.51) which is consist to previous findings \cite{meta_dataset}. However, Retriever\_Span achieves the highest score on the source domain (97.08), which is desirable because we want the best performance when there is enough annotated data. 

%\dy{should we make this a separate subsection? Or should we move this to before the Results without re-training subsection?}
%Comparing different support set, results show that Retriever\_Span model benefits from having a large support set (\texttt{support\_set=all}) for the source domain where there are 100 examples per intent, but at the same time, because examples from the target domains are much less than that from the source domains, prediction accuracy on the target domain is low. If we change the number of examples per intent from the source domain from 100 to the same as the few-shot number in the target domain (\texttt{support\_set=few}), the performance on the target domain increases dramatically but the performance on the source domain does not degrade by much. This shows that we can reduce the size of the support set to increase performance on the target domains without sacrificing performance on the source domains. 
%Furthermore, if the support set only consists of examples from the target domain (\texttt{support\_set=tgt}), the results sever as an upper-bound as there is no distraction from the source domain examples. 
%Comparing support\_set=few and support\_set=tgt, results suggest that similar to what we found in our error analysis, the major reason for incorrect prediction is that the most similar example for some queries in the target domain are from the source domains. 

% BERT has forgetting issue if not trained on source domains
% Proto_Span and Retriever_Span has no forgetting problem
% They will 
%\zy{It's quite hard to get key observations in the current version. Try starting with some highlights and then discussing each observation in one paragraph. Make it clear what each paragraph is about.}
\paragraph{Data for fine-tuning}
The \textit{Fine-tune on tgt domain} section in Table~\ref{clinc_results} shows different model behaviors when fine-tuned on the target domain data directly. 
While \texttt{BERT fine-tune} achieves high accuracy (78.89\%) on the target domain, it suffers from catastrophic forgetting on the source domain (43.91\%).
On the other hand, \texttt{Proto} and \texttt{Retriever} can get high accuracy on the target domain (80.44\% and 79.20\%) while maintaining high performance on the source domain.  

When we combine data from the source domain, we observe performance gains in all the models under the \textit{Fine-tune on tgt domain with src data} section.
%Specifically, we created a balanced dataset for all intents with few-shot examples for BERT fine-tune. Results show that \texttt{BERT} fine-tune achieves better overall accuracy (87.45\% in the avg column).
Specifically, we add few-shot source domain examples as contrastive examples for the models to learn better utterance/class representations for \texttt{Retriever} and \texttt{Proto}. 
Results show that accuracy on the target domain increases by over 3\% compared to only using target domain data.
%This shows that different from previous retrieval-based methods such as $k-$NN which require a large support set to guarantee prediction accuracy, \texttt{Retriever} is effective.
This suggests that unlike other retrieval-based methods such as $k$NN, \texttt{Retriever} does not require a large support set to guarantee prediction accuracy.
%We also note that its performance on the source domain drops slightly as we only train the model to distinguish target domain from the source domain intents, but do not re-train the model with the source domain data.


% To deal with the catastrophic forgetting problem, we multi-task target domain data with all the data from the source domain (\texttt{BERT  FT all}) or a balanced few-shot examples from each intent in the source domain (\texttt{BERT FT few}).
% Results suggest that combing all source domain data remains its performance on the source domain, but the model is optimized not only with the target domain data so that the performance on the target domain drops (64.69). In addition, it is not always practical to have all data from source domain available when we do adaptation to new domains. If we sample few-shot number of examples from the source domain instead, BERT fine-tune achieves better average performance between target and source domains although the accuracy on the target domain drops.

% \lh{The paragraph below is hard to understand}
% On the other hand, we can achieve higher accuracy for \texttt{Proto\_Span} and \texttt{Retriever\_Span} without forgetting problems on the source domain if we fine-tune directly on the target domain. 
% However, as Equation \ref{eqa:prob} shows, our batch softmax training objective it to distinguish utterance representations of different labels so that the model can only distinguish examples in the target domain without data from the source domain as negative examples. Hence, models trained this way cannot distinguish examples from the source domain so that a query in the target domain is likely to be distracted and retrieve the most similar example from the source domain. Therefore, we randomly sample the same number of examples per intent from source domain as that from the target domain during fine-tuning similar to \texttt{BERT FT few}. 


% In specific, for BERT fine-tune, in addition to directly fine-tune the model on the target domain (\texttt{BERT FT tgt}),
% we also multi-task target domain data with all the data from the source domain (\texttt{BERT  FT all}) or few-shot sample few-shot number of examples from each intent in the source domain (\texttt{BERT FT few}) to deal with the catastrophic forgetting problem.
% we also combine all the data from the source domain (\texttt{all}\xd{did this ``all'' appear in any table?}) or sample few-shot number of examples from each intent in the source domain (\texttt{src}) together with the target domain training data to solve the catastrophic forgetting problem.

% Similarly, for Proto and Retriever, we also add source domain data but with different motivations. As Equation \ref{eqa:prob} shows, our batch-softmax training objective it to distinguish utterance representations of different labels so that the model can only distinguish examples in the target domain without data from the source domain as negative examples. Therefore, we randomly sample the same number of examples per intent from source domain as that from the target domain. However, instead of training the model with the combined dataset as in BERT fine-tune, we only update the encoder parameters with the gradient from examples in the target domain. In other words, the embeddings $X$ now is the concatenation of $X_{tgt}$ and $X_{src}$ and instead of using the whole similarity matrix $S$ for training, we only use $S_{:m}$ where $m$ is the number of examples from the target domain in a batch. \dy{this part can be confusing? Reviewers may ask why we don't finetune with the src domain data (answer: the source domain can be large so that it can be expensive to include source domain data in finetuning)}

% If we further fine-tune the pre-trained model on the target domain without source domain data, BERT fine-tune can reach a high accuracy (78.89) on the target domain but suffers from catastrophic forgetting problems on the source domain (43.91).
% On the other hand, we can achieve higher accuracy for Proto and Retriever\_Span without such forgetting problems on the source domain. However, as Section \ref{exp:intent_eval} suggests, models trained this way only distinguish examples from the target domain, but cannot distinguish examples from the source domain so that a query in the target domain is likely to be distracted and retrieve the most similar example from the source domain. Therefore, we add source domain data to the target domain data during fine-tuning. 

% In specific, for BERT fine-tune, combing all source domain data remains its performance on the source domain, but the model is optimized not only with the target domain data so that the performance on the target domain drops (64.69). In addition, it is not always practical to have all data from source domain available when we do adaptation to new domains. If we sample the same few-shot number of examples from the source domain during fine-tuning, BERT fine-tune achieves better average performance between target and source domains.
% For Proto and Retriever, accuracy on the target domain also increases by a large margin (from 79.2 to 84.95) compared to using target domain data only. Particularly, Retriever\_Span achieves higher accuracy on both the target and source domains than Proto. More importantly, this shows that different from previous retrieval-based methods such as k-nearest neighbor which require a large support set to guarantee prediction accuracy, our proposed retrieval method is effective.
% We also note that performance on the source domain drops slightly because we only train the model to distinguish target domains from the source domains, but not the other way around. The model is not updated using source domain data which only serves as negative examples for target domain data. This causes the model to retrieve examples from the target domains for a query in the source domain, resulting lower accuracy (95.41 compared to 97.08).

% \paragraph{Varying the support set at inference data.}
% Another observation is that when comparing between full support sets (\texttt{support\_set=all}) and balanced support sets (\texttt{support\_set=few}), Retriever\_Span achieves higher accuracy on source domains (97.08\% vs. 95.44\%) while lower on target domains (62.69\% vs. 75.93\%). This is reasonable because full support sets have more source domain examples to increase confusion over target domains. However, this trade-off is encouraging because we can dramatically increase target domain accuracy without degrading source domain accuracy by much. \zy{I'm not sure if this is convincing because the relative reduction is similar.}

\paragraph{Impact of reduction functions} 
We compare the reduction functions proposed in Section \ref{model:train} and found that \texttt{max} performs the best.
Since \texttt{mean} is equivalent to Prototypical Networks, we compared to \texttt{Proto} directly in the experiments.
\texttt{min-max} is more intuitive in contrasting with least similar examples within the same class compared to \texttt{max}. However, its performance is worse than \texttt{max}.
% Our results show that it achieves better performance when support\_set=all, but this finding is not consistent and its performance is worse than \texttt{max} reduction function when support\_set=few.
We speculate the reason to be that 
% although the margin of the boundaries is larger, 
we retrieve the example with the maximum score at inference time so that the boundary margin may not be utilized.

%Finally, results from different data constructions are not directly comparable. For instance, constructions with larger number of intents in the source domain (and thus fewer in the target domain) generally achieve higher accuracy in the target domain. 

\input{tables/clinc_comp_results}

\paragraph{Performance over different settings}
Table~\ref{clinc_comp_results} shows the average improvement of our methods over the \texttt{BERT fine-tune} baseline, where all models are fine-tuned on the target domain with a balanced few-shot dataset after training on the source domain (same as \textit{Fine-tune on tgt domain with src data} section in Table~\ref{clinc_results}). 
Both \texttt{Proto} and \texttt{Retriever} outperforms the baseline on the target domains with a large margin, and \texttt{Retriever} has the best improvement on all intents on average.
% \texttt{Retriever} performs the best when there are relatively more data available (5-shot) whereas \texttt{Proto} performs better when there are fewer examples (2-shot). 
% Note that for 2-shot, the difference is mainly from pre-training on the source domain since \texttt{max} and \texttt{min-max} become the same for 2-shot.

%\dy{potential reason: 5-shot contains outliers to change prototype representations? A little bit hard to justify here.}

%We believe that our method can also work on open domain dialog tasks where annotations may be more scarce and other text classification tasks. We leave detailed evaluation to future work. 

\subsection{Slot Filling}
%We report our results on SNIPS in Table \ref{tab:snips_results}.
%Compared to the optimization-based method, retrieval-based models achieve higher average F1 scores, showing that deep metric learning is effective in the few-shot setting for domain adaption.
%Adding simulated transition probabilities (CDT) further improves the model performance.
%For our proposed span-level retrieval models, training the encoder on the source domain achieve better performance than directly using BERT initial checkpoint (\texttt{SimRetriever\_Span}), which demonstrates that our model is sufficient in learning label-related semantics. 
%The results also show that \texttt{Retriever\_Span} outperforms \texttt{Proto\_Span} by 17.49 after training. We conjecture that this is caused by \textt{Proto\_Span} learning noisy prototype when data is scarce, which can be justified by that the average number of examples for ATP, FSE, and SCW is small in the support set data construction shown in Appendix \ref{app:snips_details} where the difference between Proto\_Span and Retriever\_Span is large. 

% \zy{For BERT fine-tune, I'd directly call it BERT fine-tune or classification-based method. Optimization-based is a bit confusing because all methods are trained, thus optimized.}
% Table \ref{tab:snips_results} summarizes the results of our methods and baselines on SNIPS. Our span-level method (\texttt{Retriever\_Span}) achieves higher averaged F1 than all five baselines, outperforming the strongest token-level retrieval method (\texttt{L-TapNet+CDT+proto}) by 4.45\%. This shows that our model can actually predict span boundaries reliably. 
% More importantly, the better performance suggests that our span-level retrieval model is more efficient at capturing span structures compared to simulated dependencies as our method doesn't suffer from the potential discrepancy in the transition probabilities between the target and source domains. 
% We note that our method \texttt{Retriever} outperforms the strongest baseline on five out of seven domains, but has a low score on the SCW domain. We believe that this is due to the bigger difference between the test (SCW) and the development domain (GW) including the size of the support set and their respective slot names.
We note that \texttt{Retriever} outperforms the strongest baselines but reaches a low score on the SCW domain. This may be due to the bigger difference between the test (SCW) and the development domain (GW) including the size of the support set and their respective slot names.
% This makes the choice of threshold to filter spans pragmatic, which is critical in our decoding process.
We also found that from all the correctly predicted slot spans, 96.73\% predicted the correct slot names. This shows that the majority of the errors come from querying with invalid spans. We believe that span-based pre-training such as Span-BERT \cite{joshi-etal-2020-spanbert} could make our proposed method achieve better results.

% \dy{should we use ``Retriever vs. Proto'' instead? Prototypical is not really retrieval since it does not ``retrieve'' anything. Also, we didn't use ``example-based'' method in the paper}
\paragraph{Analyzing \texttt{Proto}} 
From Table~\ref{tab:snips_results}, \texttt{Retriever} outperforms \texttt{Proto} by 17\% when training the span representations.
We conjecture that this is caused by \texttt{Proto} learning noisy prototype.
Compared to \texttt{Retriever}, the similarity scores between the spans and their corresponding class representations are low, indicating that the span-level prototypes may not be clearly separated.

% when data is scarce, which can be justified by that the average number of examples for ATP, FSE, and SCW is small in the support set data construction shown in Appendix \ref{app:snips_details} where the difference between \texttt{Proto\_Span} and \texttt{Retriever\_Span} is large. 

%\dy{I moved this part from experiment here. It sounds a bit werid since we are introducing new baselines.}
%\zy{Need to revise the following paragraph}

%To compare span-level with token-level retrieval models, Retriever\_Span outperforms previous state-of-the-art L-TapNet + CDT + proto without pairwise embedding by 4.45 on F1. 
%This shows that even though we do not learn span boundaries explicitly, our model can actually predict the boundaries through span semantics. More importantly, the better performance suggests that our span-level retrieval model is more efficient in learning span and structured prediction compared to simulated dependencies where there is discrepancy between the transition probability in the target and source domains. We also note that our method Retriever\_Span outperform the strongest baseline on five out of seven domains, but receives low score on SCW domain. We believe that the difference between the test (SCW) and the development domain (GW) including the size of the support set and respective slot names makes the choice of threshold to filter spans pragmatic, which is critical in our decoding process.

\input{tables/snips_beam}

\paragraph{Ablation on decoding method}
Table \ref{snips_beam} compares beam search to greedy search. Results suggest that beam search with larger beam sizes achieve better F1 scores.
%
%\paragraph{Impact of Span Merge} 
%\zy{I removed some of the error analysis because I think it's more important to emphasize why we do span merging. We could have another paragraph for error analysis if needed.} 
As discussed in Section~\ref{sec:inference}, we merge same-label spans during inference based on a score threshold. As shown in Table \ref{snips_beam}, merging spans results in a 1.67\% F1 gain (70.43\% vs 72.10\%) under the same beam size.

% \paragraph{Error Analysis from span boundaries}

%\dy{actually, I think this should be Error Analysis since Span Merge results justify the one of the two problems}
\paragraph{Error Analysis}
We find that the main problem of our proposed model is that tokens surrounding the gold span may contain excessive contextual information so that these surrounding invalid spans retrieve corresponding spans with high similarities. For instance, in the query ``add my track to old school metal playlist'', the token ``playlist'' retrieves an actual playlist span with a high similarity score. Another major issue is that the similarity score retrieved by a partial of the gold span sometimes is higher than that retrieved by the whole span. Our ablation results on merge threshold shown in Table \ref{snips_beam} also suggest that partial spans may retrieve complete spans individually so that if we merge consecutive spans with the same slot name, we can achieve higher F1 scores.
% only 2 utterances from all the data have consecutive spans with the same slot name.

%Finally, we believe that span-based pre-training such as SpanBERT \cite{joshi-etal-2020-spanbert} can obtain better performance with our proposed methods. We use BERT embeddings in this paper to compare with previous work which mostly uses BERT as the initial checkpoint for fair comparisons.  

% \input{tables/clinc_results}



% \subsection{Benefits of Retriever}
% In addition to being more robust against overfitting and catastrophic forgetting problems, which are essential in few-shot learning settings, our proposed method has multiple advantages overs strong baselines. For instance, if the scheme is changed or some prediction bugs need to be fixed, there is minimum re-training required. More importantly, compared to classification or Prototypical Networks which require adding arbitrary number of instances to the training data and hope that the model will predict as expected \cite{yu-etal-2019-gunrock, liang-etal-2020-gunrock}, \texttt{Retriever} can guarantee the prediction when a similar query is encountered. At the same time, \texttt{Retriever} is more interpretable where the retrieved examples can serve as explanations. In addition, different from the simplified assumption that one utterance may only have one intent \cite{dit++, yu2019midas}, \texttt{Retriever} can be used to predict multiple labels. Lastly, because \texttt{Retriever} does not need to model transition probability, the decoding procedure can be paralleled and potentially be modified to be non-autoregressive for speedup. 

==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/conclusion.tex <==
\section{Conclusion}
In this paper, we propose a retrieval-based method, \texttt{Retriever}, for few-shot intent classification and slot filling. 
%We show the benefits of retrieval-based methods compared to optimization-based methods and other deep metric learning models for both practical concerns and performance.
We conduct extensive experiments to compare different model variants and baselines, and show that our proposed approach is effective in the few-shot learning scenario.
We believe that our method can also work on open domain dialog tasks where annotations may be more scarce and other text classification tasks.
In the future, we plan to extend our method to predict more complex structures with span-based retrieval. 
%For future work, we plan to extend our method to  \cite{andreas-etal-2020-task} . 

==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/ethics.tex <==
\section{Ethical Considerations}
Our intended use case is few-shot domain adaption to new classes. 
Our experiments are done on English data, but the method is not English-specific.
We use 8 Cloud TPUs V2 cores\footnote{https://cloud.google.com/tpu} for training and one V100 GPU for inference.
Since our model does not have to be retrained for the new domains, it can reduce the resources needed when applying such systems.
We claim that our proposed method outperforms baselines on few-shot slot filling and intent classification examples. Our experiments mainly focus on the 5-shot setting and the 2-shot setting, which are typical testing scenarios applied by previous work with the same claim.
    
% \begin{itemize}
%     \item Our experiments are done on English data. But the method isn't English-specific. 
%     \item We use GPUs for training the retrieval model. 
%     \item Do the claims in the paper match the experimental results, in terms of how far the results can be expected to generalize? We claim that our proposed method outperforms baselines on few-shot slot filling and intent classification examples. Our experiments mainly focus on the 5-shot setting and the 2-shot setting, which are typical testing scenarios applied by previous work with the same claim. Therefore we believe our claims match the experimental results in terms of generalization.
%     %\item Does the paper describe the steps taken to evaluate the quality of the dataset? \zy{The quality of the dataset?} The datasets we used in this paper have been standard benchmarks for these tasks and have been extensively used in previous work for comparisons.
% \end{itemize}

%PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN PLEASE FILL THIS IN 

==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/experiments.tex <==
\input{tables/clinc_results}

\section{Experiments and Results}
We evaluate our proposed approach on two datasets: CLINC \cite{larson-etal-2019-evaluation} for intent classification and SNIPS \cite{coucke-etal-2018-snips} for slot filling. Note that we use \textit{max} (Eq.~\ref{eqa:max}) as the reduction function for both tasks since it empirically yields the best results. The effect of reduction functions will be analyzed later in Section~\ref{ana:intent}.
%We use \textit{max} as our reduction function for both tasks and study \textit{min-max} for intent classification. \dy{does this sound weird?} 
%\xd{Specifically, for slot filling, we use max (Equation X) as the reduction function; for intent classification, we investigate both max and min-max (Equation X). Did you give explanation elsewhere, for why you use only use max for both, and min-max for only intent?}
%\dy{question: where should we explain that we did detailed study on intent but not slot filling (e.g. reduction function) because min-max doesn't work well so we just use max for slot filling?}
%\lh{we can briefly mention it here and give a forward reference to section 5. Also, "we apply the same model to SNIPS" seems inaccurate because the models are pretty different.}

\subsection{Intent Classification}
%\paragraph{Dataset} 
The CLINC intent classification dataset \cite{larson-etal-2019-evaluation} contains utterances from 10 intent categories (e.g., ``travel''), each containing 15 intents (e.g., ``flight\_status'', ``book\_flight'').
% \dy{domain can be confusing here because we have been talking about "source domain" so far. Any suggestions?} \lh{I think this should be fine}
%Compared to SNIPS with seven intents which are more distinguished, this dataset is more challenging and convincing, especially for few-shot learning settings.\xd{did you add this sentence, to explain why you did not eval on SNIPS for intent? is it needed?} \lh{+1}
To simulate the few-shot scenario where new domains and intents are introduced, we designate $n_c$ categories and $n_i$ intents per category as the source domain (with all 100 training examples per intent), and use the remaining $150 - n_c \times n_i$ intents as the target domain. We experiment with $(n_c, n_i) = (10, 10)$, $(8, 10)$, and $(5, 15)$.
\footnote{ $(n_c, n_i) = (10, 10)$ simulates the situation where all the categories are known, but we adapt to new intents in all 10 categories; $(n_c, n_i) = (5, 15)$ simulates the situation where we adapt to 5 entirely new intent categories.}
The target training data contains either 2 or 5 examples per target intent.
% Domains and intents in each domain are randomly sampled.

% \paragraph{Settings}
We compare our proposed method \texttt{Retriever} with
a classification model \texttt{BERT fine-tune} and a Prototypical Network model \texttt{Proto}. The former learns a linear classifier on top of BERT embeddings~\cite{devlin-etal-2019-bert}, and the latter learns class representations based on Prototypical Networks.\footnote{Previous work show that Prototypical Networks outperforms other optimization-based and metric-learning models such as MAML in (intent) classification tasks \cite{meta_dataset, krone-etal-2020-learning}.} We also show results with the initial BERT checkpoint without training ($\texttt{Proto}^{\texttt{frz}}$, $\texttt{Retriever}^{\texttt{frz}}$). We use the same batch size for all models, and tune other hyperparameters on the development set before testing. 

\paragraph{Evaluation}
\label{exp:intent_eval}
%\xd{I think this paragraph is a little confusing, maybe refer to how previous few-shot intent work write the eval description section? like what you did for slot filling evaluation details paragraph (following Hou et al., 2020...).}
We sample domains and intents three times for each $(n_c, n_i)$ setting, and report average prediction accuracy.
We report accuracy on intents from the target domain ({tgt}), source domain ({src}), and the macro average across all intents ({avg}).

In addition to applying the model to the target domain after pre-training on the source domain without re-training (\textit{Pre-train on src domain}), we also evaluate the model performance with fine-tuning. We re-train the model with either target domain data only (\textit{Fine-tune on tgt domain}) or a combination of source and target domain data (\textit{Fine-tune on tgt domain with src data)}.

Moreover, we evaluate the models with the following support set variations: 
with target domain data and all data in the source domain ({support\_set=all}), 
with equal number of examples (same as the few-shot number) per intent ({support\_set=balance}),
and with only examples from the target domain ({support\_set=tgt}). The last one serves as an upper-bound for the target domain accuracy.

\input{tables/snips_results}

\paragraph{Results}
Table \ref{clinc_results} shows the results for $(n_c, n_i) = (10, 10)$ and 5 examples per target intent; results on other settings exhibit the same patterns (See Appendix~\ref{app:clinc_results}). We observe that \texttt{Retriever} performs the best on the source domain (97.08\%) before fine-tuning. \texttt{Retriever} also achieves the highest accuracy on the target domain (84.95\%) after fine-tuning, while maintaining competitive performance on the source domain (95.41\%) among all the methods. %\zy{Maybe also emphasize that the accuracy on the source domain is also competitive so we have a single model that achieves the best of both worlds.}



\subsection{Slot Filling}
%\paragraph{Dataset} 
SNIPS \cite{coucke-etal-2018-snips} is a slot filling dataset containing 39 slot names from 7 different domains: GetWeather (GW), PlayMusic (PM), AddToPlaylist (ATP), RateBook (RB),  FindScreeningEvent (FSE), BookRestaurant (BR), and SearchCreativeWork (SCW).
%Following the data split provided by \citet{hou-etal-2020-shot}, for each testing domain, we choose one domain for development and use the rest five domains for training the model.\xd{maybe first mention we train on utterances from 5 out of 7 domains, and test on the 7th domain.} 
Following \citet{hou-etal-2020-shot}, we train models on five source domains, use a sixth one for development, and test on the remaining domain.
%Since one utterance can have different numbers of instances for each slot name, the $K$-shot support set consists of minimum number of utterances where there are at least $K$ instances for each slot name.\xd{this sentence is understandable with some efforts} \dy{is it clear that we use the the data provided by Hou et al. 2020 here?}
We directly use the $K$-shot split provided by \citet{hou-etal-2020-shot}, where the support set consists of the minimum number of utterances such that at least $K$ instances exist for each slot name.
We also set $K = 5$ in our experiment.
Appendix~\ref{app:snips_details} contains further details about the setup.

%Table~\ref{tab:snips_results} shows results on the setting of $K=5$.
% Results for $K=2$ have similar performance patterns, and are omitted due to space limit.\lh{Can we put them in the Appendix?}
%Since our proposed method requires positive examples during training similar to duel encoder models \cite{yang-etal-2019-improving} such that $K \geq 2$, we evaluate all the models with 5-shot support sets.

%\paragraph{Baselines}
%\texttt{BERT fine-tune} is an optimization-based model which fine-tunes BERT NER models \cite{devlin-etal-2019-bert} on the testing domain after pre-training on the source domain. On token-level Retriever initialized with BERT embeddings, \texttt{SimBERT} retrieves the most similar token using cosine similarity without fine-tuning, and \texttt{Matching} uses Matching Networks \cite{vinyals-etal-2016-matching} while \texttt{Proto} leverages Prototypical Networks \cite{snell-etal-2017-prototypical} to learn label representations. We also compare with CDT based on a CRF framework proposed by \citet{hou-etal-2020-shot} with label-enhanced Prototypical Networks (\texttt{L-Proto + CDT + pair-wise}) and TapNet \cite{yoon-etal-2019-tapent}. 
%Note that the two CDT models combined label semantics \cite{shah-etal-2019-robust} and pair-wise embedding, which concatenates query and support utterances before generating query embedding with cross-attention. In particular, pair-wise embeddings have been shown to achieve better results than embedding query and support separately, but can be expensive both in memory and computation at inference time, especially when the number of support set is large \cite{poly_encoder}. In contrast, our proposed methods embed the support set with the trained encoder after training, and embed query utterances independently during inference before retrieving examples in the support set.
%\citet{hou-etal-2020-shot} further incorporates prototypical references into TapNet. To make fair comparisons, we only compare with \texttt{L-TapNet + CDT + proto} without pair-wise embeddings.\xd{I think there're too many details from ``Yoon et al., 2019'' to here, maybe comment some out and put some info in footnote.}
We compare against two baselines and three models from the previous work. \texttt{BERT Tagging} is a BERT-based BIO tagging model \cite{devlin-etal-2019-bert} fine-tuned on the testing domain after training on the source domains, while $\texttt{SimilarToken}^{\texttt{frz}}$ uses BERT embeddings to retrieve the most similar token based on cosine similarity without any training. 
\texttt{MatchingToken} and \texttt{ProtoToken} are two token-level methods that leveraged Matching Networks \cite{vinyals-etal-2016-matching} and Prototypical Networks \cite{snell-etal-2017-prototypical} 
% to learn label representations 
respectively.
\texttt{L-TapNet+CDT+proto} \cite{hou-etal-2020-shot} is an adaptation of TapNet \cite{yoon-etal-2019-tapent} with label semantics, CDT transition probabilities, and Prototypical Networks.
% \texttt{BERT fine-tune} is a BERT-based BIO tagging model \cite{devlin-etal-2019-bert} fine-tuned on the testing domain after pre-trained on the source domains,
% %Secondly, we compare with a token-level Retriever baseline, 
% while \texttt{SimBERT} uses BERT embeddings to retrieve the most similar token based on cosine similarity without further fine-tuning. 
%The rest of the three baselines are previous work that achieved competitive or state-of-the-art performance on this task.  \cite{yoon-etal-2019-tapent} to the slot filling task.


% Note that \citet{hou-etal-2020-shot} showed that adding pair-wise embeddings with cross-attention yielded much better performance. However, this method is expensive both in memory and computation at inference time comparing to independent embeddings, and it can be infeasible if the support set is large \cite{poly_encoder}. For reference, we show the most accurate models in Table \ref{tab:snips_results}, referred as \texttt{L-Proto + CDT + pair-wise} and \texttt{L-TapNet + CDT + Proto + pair-wise}. Our method which pre-computes support example embeddings and only compute query embeddings at inference time even outperforms \texttt{L-Proto + CDT + pair-wise} with less memory and computation cost. \dy{shouldn't we talk about this in the results section rather than here?} \zy{Yeah I agree. I feel even the whole paragraph can be in the results because they are not really baselines.} For fair comparison, we do not compare directly with \texttt{L-TapNet + CDT + Proto + pair-wise}, which also includes a Proto component.

%\paragraph{Our method}
% We experiment with several variants of our proposed method. 
% \texttt{Proto\_Span} retrieves the most similar slot prototype, while \texttt{Retriever\_Span} retrieves the most similar slot example. 
% Similar to \texttt{SimBERT}, \texttt{SimProto\_Span} and \texttt{SimRetriever\_Span} does Retriever on with BERT encodings without any target domain finetuning.

% The Retriever models are trained on source domains (unless otherwise noted) and early stopped based on metrics on the development domains.
% %before being evaluated on the testing domains.
% %without further fine-tuning. 

We experiment with several variants of our proposed method. \texttt{Proto} trains Prototypical Networks to compute span class representations. \texttt{Retriever} retrieves the most similar slot example for each span. Both methods use the same decoding method. Similar to $\texttt{SimilarToken}^{\texttt{frz}}$, $\texttt{Proto}^{\texttt{frz}}$ and $\texttt{Retriever}^{\texttt{frz}}$ use the original BERT embeddings without any training.
% 
% Unless otherwise noted, 
All models are trained on source domains and early stopped based on performance on the development domains.



\paragraph{Evaluation}
We report F1 scores for each testing domain in a cross-validation episodic fashion. 
Following \citet{hou-etal-2020-shot}, we evaluate each testing domain by sampling 100 different support sets and ten exclusive query utterances for each support set. We calculate F1 scores for each episode and report average F1 scores across 100 episodes.

\paragraph{Results}
Table \ref{tab:snips_results} summarizes the experiment results on the SNIPS dataset. Our span-level method (\texttt{Retriever}) achieves higher averaged F1 than all five baselines, outperforming the strongest token-level method (\texttt{L-TapNet+CDT+proto}) by 4.45\%. This shows that our model is effective at span-level predictions. 
More importantly, the better performance suggests that our span-level \texttt{Retriever} model is more efficient at capturing span structures compared to simulated dependencies as our method does not suffer from the potential discrepancy in the transition probabilities between the target and source domains. 
% \lh{Do we have qualitative analysis to back this up?}
% \dy{re: I couldn't find examples from previous work }

Although~\citet{hou-etal-2020-shot} showed that adding pairwise embeddings with cross-attention yielded much better performance, this method is expensive both in memory and computation at inference time, especially when the support set is large~\cite{poly_encoder}.
%For reference, we show the most accurate models in Table \ref{tab:snips_results}, referred as 
For fair comparison, we do not directly compare with methods using pairwise embeddings (methods with $^\texttt{pw}$ in Table~\ref{tab:snips_results}).
%$\texttt{L-Proto+CDT}^\texttt{pw}$ and $\texttt{L-TapNet+CDT+Proto}^\texttt{pw}$. 
Note that our method with pre-computed support example embeddings even outperforms $\texttt{L-Proto+CDT}^\texttt{pw}$ with less memory and computation cost. 
%For fair comparison, we do not directly compare with $\texttt{L-TapNet+CDT+Proto}^\texttt{pw}$, which also includes a Proto component.




% \input{tables/snips_beam}

% \input{tables/snips_merge}




% \xd{column 1\&4 in table 3?}, 
% \xd{column3\&6?}.
% on three different data splits for each data construction
%\dy{is this clear? we sample data three times and report the average for each data construction}. 
% Different from slot filling where we only evaluate the models without re-training on the target domain to be consistent with previous research, we also evaluate all models with fine-tuning on the target domain after pre-training on the source domain for intent classification. In specific, for BERT fine-tune, in addition to directly fine-tune the model on the target domain (\texttt{BERT FT tgt}),
% we also multi-task target domain data with all the data from the source domain (\texttt{BERT  FT all}) or few-shot sample few-shot number of examples from each intent in the source domain (\texttt{BERT FT few}) to deal with the catastrophic forgetting problem.
% % we also combine all the data from the source domain (\texttt{all}\xd{did this ``all'' appear in any table?}) or sample few-shot number of examples from each intent in the source domain (\texttt{src}) together with the target domain training data to solve the catastrophic forgetting problem.

% Similarly, for Proto and Retriever, we also add source domain data but with different motivations. As Equation \ref{eqa:prob} shows, our batch-softmax training objective it to distinguish utterance representations of different labels so that the model can only distinguish examples in the target domain without data from the source domain as negative examples. Therefore, we randomly sample the same number of examples per intent from source domain as that from the target domain. However, instead of training the model with the combined dataset as in BERT fine-tune, we only update the encoder parameters with the gradient from examples in the target domain. In other words, the embeddings $X$ now is the concatenation of $X_{tgt}$ and $X_{src}$ and instead of using the whole similarity matrix $S$ for training, we only use $S_{:m}$ where $m$ is the number of examples from the target domain in a batch. \dy{this part can be confusing? Reviewers may ask why we don't finetune with the src domain data (answer: the source domain can be large so that it can be expensive to include source domain data in finetuning)}

==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/figures/intro_figure.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=0.9\textwidth]{span_retrieval.pdf}

\caption{Illustration of span-level retrieval for slot filling. 
% \lh{make numbers bigger maybe?} 
For each span (including spans that are not valid slots such as \textit{``book a table''}) in the input utterance, we retrieve its most similar span
%representation in the support data indexed by contextual embedding
from the retrieval index,
and then assign the slot name as the prediction with a similarity score. We use modified beam search to decode an output that maximizes the average similarity score. 
The gold slots are \textit{``black horse tavern''} and \textit{``7 pm''} in this example.
%and extract the spans ``black horse tavern'' of ``restaurant\_type'' and ``7 pm'' of ``time\_range'' slot names. For intent classification, we use the [CLS] token to retrieve the most similar utterance in the support set.
% \lh{there are lot going on in the figure. maybe drop the CRF/BIO-tagging part? It might confuse readers and make them think we are doing BIO tagging ...}
% \xd{This simplified version is better. why does ``black’’ receive relatively high score and why is  ``book a table’’ most similar to ``walking distance’’, shouldn’t it be ``book a taverna’’? I think you don’t need to use exactly the same example and predictions in the dataset in Figure 1 —  to make it easier to understand is more important.}
}
\label{fig:illustration}
\vspace{-1em}
\end{figure*}

==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/introduction2.tex <==
\section{Introduction}

\input{figures/intro_figure}

Few-shot learning is a crucial problem for practical language understanding applications.
In the few-shot setting, the model (typically trained on source domains with abundant data) needs to adapt to a set of unseen labels in the target domain with only a few examples. For instance, when developers introduce a new product feature, a query understanding model has to learn new semantic labels from a small dataset they manage to collect.

Few-shot learning is challenging due to the imbalance in the amount of data between the source and target domains.
Traditional classification methods,
% ~\cite{mesnil-etal-2014-using, lample-etal-2016-neural, goo-etal-2018-slot}
even with the recent advancement of
pre-trained language models~\cite{peters-etal-2018-deep, devlin-etal-2019-bert}, could suffer from over-fitting~\cite{snell-etal-2017-prototypical, meta_dataset} or catastrophic forgetting~\cite{wu-etal-2019-transferable}
when incorporating the data-scarce target domain.
%
On the other hand,
\emph{metric learning methods} \cite{weinberger-etal-2006-distance, vinyals-etal-2016-matching, snell-etal-2017-prototypical} %are well-suited for few-shot scenarios. 
have been shown to work well in few-shot scenarios.
These methods are based on modeling similarity between inputs, effectively
%, rather than task-specific classifiers. 
allowing the model to be decoupled from the semantics of the output space. For example, a model would learn that the utterance \textit{``I'd like to book a table at black horse tavern at 7 pm''} (from Figure~\ref{fig:illustration}) is similar to \textit{``make me a reservation at 8''} and thus are likely to have similar semantic representations, even without knowing the semantic schema in use.
Unlike learning output labels, which is difficult when examples are scarce,
learning a similarity model can be done on the abundant source domain data, making such models data-efficient even in few-shot settings.
%Thus, these methods are less susceptible to data imbalance between the source and the target domains and catastrophic forgetting in the few-shot scenarios~\cite{snell-etal-2017-prototypical, meta_dataset}.

While there are many instantiations of metric learning methods (see Section~\ref{sec:related}), we focus on \emph{retrieval-based} methods, which maintain an explicit retrieval index of labeled examples. The most basic setting of retrieval-based model for few-shot learning is: after training a similarity model and encoding target domain data into the index, we can retrieve examples most similar to the given input, and then make a prediction based on their labels.
% (e.g., by majority voting). 
Compared to methods that do not maintain an index, such as Prototypical Networks
% \dy{should we say ``compared to methods that rely on class representations'' instead of ``that do not maintain an index''?}\zy{I feel ``maintain an index'' is more consistent with the sentences above. or sth like ``do not rely on example-based retrieval'' }
\cite{snell-etal-2017-prototypical}, retrieval-based methods
% Compared to other metric learning methods such as Prototypical Networks \cite{snell-etal-2017-prototypical} with prototype representations, retrieval-based methods classify a query to its most similar example. They
are less sensitive to outliers with few data points, and are powerful when we have abundant data in the source domain \cite{meta_dataset}. 
% Moreover, a retrieval-based model can be applied to new domains even without retraining the similarity model. 

% \lh{cite some related work}
%Moreover, they allow one to exploit the power of pre-trained language models, making it promising for few-shot learning settings.
%
% Therefore, retrieval-based methods have been a popular choice for few-shot intent classification tasks.
% Moreover, text similarity models also allows one to exploit the power of pre-trained language models. For example, the freezed BERT model can already do reasonably well. Recent GPT-3~\cite{brown-etal-2020-langauge} results also illustrate the potential of few-shot and zero-shot capability.

However, applying retrieval-based models on tasks with a structured output space is non-trivial.
%For example, given the queries shown above, a slot-filling model needs to predict that the \texttt{time} for the booking as \textit{``7 pm''} and \textit{``8''}, respectively, and that the \texttt{restaurant} in the first query as ``black horse tavern''.
For example, even if we know that the utterance in Figure~\ref{fig:illustration} is similar to \textit{``make me a reservation at 8''}, we cannot directly use its slot values (e.g., the \texttt{time} slot has value \textit{``8''} which is not in the input), and not all slots in the input (e.g., \textit{``black horse tavern''}) have counterparts in the retrieved utterance.
While previous works have exploited token-level similarity methods in a BIO-tagging framework, they had to separately simulate the label transition probabilities, which might still suffer from domain shift in few-shot settings~\cite{wiseman-stratos-2019-label, hou-etal-2020-shot}.

In this work, we propose \texttt{Retriever}, a retrieval-based framework that tackles both classification and span-level prediction tasks. 
%\ice{retrieval-based method comes very late. Like Terry said, we should motivate retrieval a lot more}
%, which classifies queries to their most similar labeled examples from a few-shot support set.
The core idea is to match \emph{token spans} in an input to the most similar labeled spans in a retrieval index.
%Compared to other metric learning methods such as Prototypical Networks \cite{snell-etal-2017-prototypical}, retrieval-based methods are less sensitive to outliers with few data points, and are powerful when we have abundant data in the source domain \cite{meta_dataset}. 
%In addition, they are appealing for hot fix since new data can be added without retraining and they are also more interpretable.
%We apply such models not only to the full input texts, but also spans in the text. 
For example, for the span \textit{``7 pm''} in the input utterance, the model retrieves \textit{``8''} as a similar span (given their surrounding contexts), thus predicting that \textit{``7 pm''} has the same slot name \texttt{time} as \textit{``8''}.
During training, we fine-tune a two-tower model with BERT \cite{devlin-etal-2019-bert} encoders, along with a novel batch softmax objective, to encourage high similarity between contextualized span representations sharing the same label.
At inference time, we retrieve the most similar span from the few-shot examples for every potential input span, and then decode a structured output that has the highest average span similarity score.

We show that our proposed method is effective on both few-shot intent classification and slot-filling tasks, when evaluated on CLINC~\cite{larson-etal-2019-evaluation} and SNIPS~\cite{coucke-etal-2018-snips} datasets, respectively. 
Experimental results show that \texttt{Retriever} achieves high accuracy on few-shot target domains without retraining on the target data. For example, it outperforms the strongest baseline by 4.45\% on SNIPS for the slot-filling task.

% SNIPS \cite{coucke-etal-2018-snips} slot filling task. 
% We also show that the same approach works for intent classification on the CLINC \cite{larson-etal-2019-evaluation} dataset. 
%\lh{Add sth. about results}
%Analysis results show that ?????



\section{Benefits of Retriever}
In addition to being more robust against overfitting and catastrophic forgetting problems, which are essential in few-shot learning settings, our proposed method has multiple advantages overs strong baselines. For instance, if the scheme is changed or some prediction bugs need to be fixed, there is minimum re-training required. More importantly, compared to classification or Prototypical Networks which require adding arbitrary number of instances to the training data and hope that the model will predict as expected \cite{yu-etal-2019-gunrock, liang-etal-2020-gunrock}, \texttt{Retriever} can guarantee the prediction when a similar query is encountered. At the same time, \texttt{Retriever} is more interpretable where the retrieved examples can serve as explanations. In addition, different from the simplified assumption that one utterance may only have one intent \cite{dit++, yu2019midas}, \texttt{Retriever} can be used to predict multiple labels. Lastly, because \texttt{Retriever} does not need to model transition probability, the decoding procedure can be paralleled and potentially be modified to be non-autoregressive for speedup. We can also tune threshold (explained in Section \ref{model_slot_decoding}) to change precision and recall according to use case requirements.

==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/introduction_old.tex <==
\section{Introduction}
\lh{The intro feels a lot better length-wise. I think we probably need to work more on the motivation part.}

Few-shot learning scenarios are prevalent and are challenging to data-intensive supervised learning methods. For instance, there are constant expansions to new domains and labels to support more tasks but there may only be few annotated data points for these new labels. Motivated by this, we focus on cross-domain adaptation by training on the source domains with larger amounts of data, and then apply the trained model to the target domain with only few annotated examples on slot filling and intent classification tasks.


% Structured prediction such as slot filling and text classification such as intent classification are essential natural language understanding tasks.
% % in task-oriented dialog systems. 
% For example, in task-oriented dialog systems, given a user utterance ``I'd like to book a table at black horse tavern at 7 pm'', the slot filling task is to find task-related slot values such as ``\texttt{7 pm}'' and the corresponding slot names such as ``\texttt{time range}'' in a structured prediction paradigm. The intent classification task is to classify the utterance to the ``\texttt{restaurant booking}'' class. 
% %Similarly, the intent classification task is to find the user intent for the whole utterance. 
% In virtual assistants such as Alexa and Google Assistant, few-shot learning scenarios are prevalent and are challenging to data-intensive supervised learning methods.
% For instance, there are constant expansions to new domains and labels during deployment to support more tasks but there may only be few annotated data points for these new labels. 
% %In addition, changing of annotation schemas such as using more fine-grained annotation can also be considered as few-shot setting. 
% Motivated by this, we focus on cross-domain adaptation by training on the source domains with larger amounts of data, and then apply the trained model to the target domain with only few annotated examples.

% Traditionally, researchers leverage linear classification models on top of neural encoders to predict BIO labels with linear conditional random fields (CRFs, \citealp{lafferty-etal-2001-conditional}) for slot filling, and to predict intent classes with a linear layer for intent classification \cite{mesnil-etal-2014-using, lample-etal-2016-neural, goo-etal-2018-slot}. Even though large language model pre-training boosts the performance on both tasks \cite{peters-etal-2018-deep, devlin-etal-2019-bert}, these models are often data intensive and do not work well for few-shot settings due to overfitting with inductive bias \cite{snell-etal-2017-prototypical, meta_dataset} and catastrophic forgetting problems on the source domain \cite{wu-etal-2019-transferable}.

Traditionally, researchers leverage linear classification models for slot filling and intent classification \cite{mesnil-etal-2014-using, lample-etal-2016-neural, goo-etal-2018-slot} and more recently, with pre-trained language models \cite{peters-etal-2018-deep, devlin-etal-2019-bert}. However, these models are often data intensive due to the bottleneck of learning linear layers for labels. Thus they suffer from overfitting with inductive bias  in few-shot settings. In addition, they are prone to catastrophic forgetting on the source domain \cite{wu-etal-2019-transferable}.

% An alternative direction is metric learning \cite{vinyals-etal-2016-matching, snell-etal-2017-prototypical} to learn embedding representations which has shown superior performance for few-shot settings in both vision and language tasks.
% Similar to GPT-3 \cite{brown-etal-2020-langauge}, these methods do not require fine-tuning the whole model on new domains which have limited annotated examples, thus are less susceptible to overfitting and catastrophic forgetting problems. More importantly, these methods decouples learned models from the semantics by only associating semantics with the retrieval index.
%, and thus are robust to schema changes and simplify point-fixing.
% Recently, metric learning methods such as Prototypical Networks \cite{snell-etal-2017-prototypical} have been applied to slot filling and intent classification tasks \cite{wiseman-stratos-2019-label, hou-etal-2020-shot, sun-etal-2019-hierarchical} and performance gains have been observed. However, they focus on token-level similarity learning and either ignore or simulate a noisy bi-gram label dependency to decode a sequence of label predictions. In addition, performance on the source domain where we have more training examples is critical, but \citet{meta_dataset} showed that these methods perform poorly in this setting compared to fine-tuning.

An alternative approach is metric learning \cite{weinberger-etal-2006-distance, vinyals-etal-2016-matching, snell-etal-2017-prototypical}. These models are usually based on similarity models rather than task-specific classifiers, allowing decoupling the learned models from the semantics by only associating semantics with the retrieval index. Since methods such as nearest neighbor retrieval map queries to the neighborhood around each support example, they are less susceptible to catastrophic forgetting and data imbalance between the source and target domains. 
These benefits make it appealing to apply to few-shot settings.
Recently, metric learning methods such as Prototypical Networks \cite{snell-etal-2017-prototypical} have been applied to slot filling and intent classification tasks \cite{wiseman-stratos-2019-label, hou-etal-2020-shot, sun-etal-2019-hierarchical}. 
However, they focus on token-level similarity learning for slot tagging and either ignore or simulate a noisy bi-gram label transition probabilities to decode a sequence of tags. 


%\lh{maybe emphasis that in previous paragraphs that most of the few-shot learning literature focus on intent classification and doesn't work well with structured prediction tasks}
In this paper, we propose to learn span-level similarity retrieval models and decode the retrieved spans to a valid structure. 
In addition to the benefits of metric learning and other non-parametric models such as GPT-3 \cite{brown-etal-2020-langauge} in the few-shot setting,
retrieval-based methods are less sensitive to outliers in prototype representations and can also perform well in large-shot settings compared to methods such as Prototypical Networks.
% we fine-tune BERT \cite{devlin-etal-2019-bert} using batch softmax to learn similar representations to spans sharing the same label with hard examples on the source domain.
\dy{does "two-tower model" indicate dual-encoder? Note that we are very different from dual encoder models}
During training, we fine-tune a two-tower model with BERT \cite{devlin-etal-2019-bert} encoders to enforce high similarity between span embeddings sharing the same label.
We introduce a novel batch softmax loss and empirically show that it performs better than other methods.
At inference time, we retrieve the most similar span from the few-shot in-domain examples to each potential span and decode a set of spans that has the maximum average similarity score.
%as the sequence prediction.
We then expand the span-level retrieval to utterance-level retrieval for intent classification. 
We show that our proposed method is effective by
evaluating it on SNIPS \cite{coucke-etal-2018-snips} for slot filling and CLINC \cite{larson-etal-2019-evaluation} for the intent classification task independently.
\dy{I focused on highlighting the benefits/motivation of using retrieval vs. prototypcal, i.e. less sensitive to outliers; work well for large-shots. However, I think the benefits of 1. interpretable 2. deterministic and hot-fix, (3. fast decoding) should also be mentioned here.}

% Moreover, our retrieval-based method is interpretable, and the prediction is deterministic once the examples are added, compared to methods such as Prototypical Networks.
% Moreover, span-level retrieval can lift the requirement of sequential dependencies and thus speed up the decoding procedure, similar to non-autoregressive slot tagging.
% We show that our proposed method is effective by
% evaluating it on SNIPS \cite{coucke-etal-2018-snips} for slot filling and CLINC \cite{larson-etal-2019-evaluation} for the intent classification task independently.

==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/model.tex <==
\section{Model}

%\lh{I think this section requires an overview before diving into "batch softmax."}
% \lh{It's also a good place to explain problem definition, input-output space, and that we are doing both intent classification and slot filling}
% For an utterance from the new domain where there are few-shot in-domain examples in the support set, we retrieve a span in the support set for each potential span and use the retrieved span label as the slot name prediction. Similarly, we retrieve the most similar utterance in the utterance level and use the retrieved utterance label as the intent prediction.
% As shown in Figure \ref{fig:illustration},
% we construct a support set with examples from both the source domains as well as the few-shot target domain.

% \eat{
% As shown in Figure \ref{fig:illustration},
% we construct a support set of $\{(x^i, y^i)_{i=1}^M\}$ where $M$ is the number of spans in the few-shot target domain examples and $(x^i, y^i)$ are (slot\_name, slot\_value) pairs.
% Given an input utterance $u$, we retrieve its most similar span representation from the support data indexed by their contextual embeddings, and then decode the final output span that maximizes average similarity scores with beam search. If we apply our method to the intent classification task, then $M$ is the number of few-shot target domain examples and $(x^i, y^i)$ are (utterance, label) pairs. 
% In our preliminary experiments, Siamese Networks and Dual Encoder Models \cite{yang-etal-2019-improving} without a classification head under-perform linear classifiers by a large margin \cite{ren-etal-2020-intention}. To combine the benefits of classifiers but eliminate the bottleneck in the linear layer for few-shot learning, we propose to use batch softmax to train our retrieval-based model without the requirement of mining hard negative pairs \cite{gillick-etal-2019-learning, zhang-etal-2018-discriminative}.
% }

% To eliminate the problems of large training pairs required and low accuracy compared to fine-tuning methods in our preliminary experiments with Siamese Networks \cite{koch-etal-2015-siamese} and Dual Encoder Models \cite{yang-etal-2019-improving}, we propose to use batch softmax to train our retrieval-based model.
%\lh{I remember we talked about citation for batch softmax, should we cite it?}
%\dy{I searched about ``batch softmax" but didn't see any result. So I don't know if people have used the exactly same softmax method before. }
%the slot filling task is to extract spans that are slot values of a set of pre-defined slot names, whereas the intent classification task is to classify the utterance to a set of intent class labels.

%%%%%%% ALTERNATIVE VERSION HERE %%%%%%%
We propose a retrieval-based model, \texttt{Retriever}, for intent classification and slot filling in the few-shot setting.
Figure \ref{fig:illustration} illustrates our approach.
At a high level, from examples $(\mathbf{x}, \mathbf{y})$ in the target training data (and optionally the source training data), we construct a retrieval index consisting of labeled spans $(r, \ell)$ from $\mathbf{y}$. Given a test utterance $\mathbf{x}$, for each span of interest in $\mathbf{x}$ (all spans $\mathbf{x}_{i:j}$ for slot filling; only $\mathbf{x}_{1:n}$ for intent classification), we retrieve the most similar labeled spans $(r, \ell)$ from the index, and then use them to decode an output $\mathbf{y}$ that maximizes the average span similarity score.

The use of retrieval provides several benefits. For instance, we empirically show in Section \ref{ana:intent} that the model does not suffer from catastrophic forgetting because both source and target data are present in the retrieval index. Class imbalance can also be directly mitigated in the retrieval index. Additionally, since the trained model is non-parametric, we could replace the retrieval index to handle different target domains without having to retrain the model. This also means that the model does not need access to target data during training, unlike traditional classification methods.

\subsection{Retriever}
\label{model:train}

The retriever is the only trainable component in our model. Given a query span $r' = \mathbf{x}_{i:j}$ from the input $\mathbf{x}$, the retriever returns a set of labeled spans $(r, \ell)$ with the highest similarity scores $s(\mathbf{z}, \mathbf{z}')$, where $\mathbf{z} = E(r)$ and $\mathbf{z}' = E(r')$ are the contextualized embedding vectors of $r$ and $r'$, respectively.
%For brevity, we might also use $\mathbf{z}$ to refer to the spans.

\paragraph{Similarity score}
To compute the contextualized embeddings $\mathbf{z}$ and $\mathbf{z}'$ of spans $r$ and $r'$, we first apply a Transformer model initialized with pre-trained BERT on the utterances where $r$ and $r'$ come from. For slot filling, we follow \citet{toshniwal-etal-2020-cross} and define the span embedding as the concatenated embeddings of the its first and last wordpieces.
For intent classification, we use the embedding of the [CLS] token.
We then define $s(\mathbf{z}, \mathbf{z}')$ as the dot product\footnote{We experimented with affine transformation as well as cosine similarity but did not see any performance gain. For intent classification, using the [CLS] token achieves better results than averaging word embeddings.}
between $\mathbf{z}$ and $\mathbf{z}'$.

\paragraph{Training with batch softmax}
% In the source domain, we have $N$ class labels $\ell_1, \ell_2, ..., \ell_N$ where each class label refers to a slot name (such as \texttt{restaurant\_name}) in slot filling or an intent (such as  \texttt{book\_flight}) for the intent classification task. 
% \zy{Clarify that we sample $b$ examples from each class in a batch.} 
We use examples from the source domain to train \texttt{Retriever}. Let $\ell_1, \dots, \ell_N$ be the $N$ class labels (slot or intent labels) in the source domain.
% For each class label, we define $e_1^1, e_1^2, ... e_1^b$ as training examples for class label $\ell_1$, 
% and $e_2^1, e_2^2, ... e_2^b$ as training examples for class label $\ell_2$, etc. Here $e$ is either a span for slot filling or an utterance for intent classification, and $b$ is the batch size per class.
To construct a training batch,
for each class label $\ell_i$, we sample $B$ spans $r_i^1, \dots, r_i^B$ from the training data with that label, and compute their embeddings $\mathbf{z}_i^1, \dots, \mathbf{z}_i^B$.
% \footnote{If the number of examples in each class is unbalanced or the number of shots is less than $b$ in a batch, then we pad each class to $b$ examples by randomly sampling examples in the class.}. 
%We encode the training examples with an encoder $E$ into $d$-dimensional embeddings $X\in\mathbb{R}^{p \times N \times d}$: 
% \begin{equation}
%     \begin{split}
%         X & = E(e_1^1, e_1^2, ..., e_1^b, e_2^1, e_2^2, ..., e_2^b, ...) \\
%           & = \mathbf{x}_1^1, \mathbf{x}_1^2, ..., \mathbf{x}_1^b, \mathbf{x}_2^1, \mathbf{x}_2^2, ..., \mathbf{x}_2^b, ...
%     \end{split}
% \end{equation}
% where $\mathbf{x}_\ell^i$ is the $i$th example in the batch with the label $\ell$.
% For slot tagging, $\mathbf{x}_\ell^i$ is the concatenated embeddings of its first and last tokens in the span following \citet{toshniwal-etal-2020-cross}.
% For intent classification, $\mathbf{x}_\ell^i$ is the embedding of the [CLS] token.
%We create a similarity matrix $S$ with a similarity function $s$ between each pair of spans in the training batch as $S = s(X, X^T) $.
% \zy{Did you use any cosine similarity or affine transformation in your experiment, or just dot product? Might be worth adding a footnote here if you found cosine similarity didn't work as good as dot product.}
% \begin{equation}
%     \begin{split}
%         S & = s(X, X^T) 
%     \end{split}
% \end{equation}
%The similarity between each example embedding $\mathbf{x}_\ell^i$ and the other examples in the same batch can be shaped as:
Then, for each query span $r_i^j$, we compute similarity scores against all other spans in the batch to form a $B\times N$ similarity matrix:
\begin{equation}
\label{eqa:matrix}
S_i^j = \begin{bmatrix}
s(\mathbf{z}_i^j, \mathbf{z}_1^1) & s(\mathbf{z}_i^j, \mathbf{z}_2^1) & \dots & s(\mathbf{z}_i^j, \mathbf{z}_N^1) \\
s(\mathbf{z}_i^j, \mathbf{z}_1^2) & s(\mathbf{z}_i^j, \mathbf{z}_2^2) & \dots & s(\mathbf{z}_i^j, \mathbf{z}_N^2) \\
\vdots & \vdots & \ddots & \vdots \\
s(\mathbf{z}_i^j, \mathbf{z}_1^B) & s(\mathbf{z}_i^j, \mathbf{z}_2^B) & \dots & s(\mathbf{z}_i^j, \mathbf{z}_N^B) \\
\end{bmatrix}.
\end{equation}
We now summarize the score between $r_i^j$ and each label $\ell_{i'}$ by applying a reduction function (defined shortly) along each column to get a $1 \times N$ vector:
\begin{equation}
\label{eqa:prob}
\hat{S}_i^j =
\begin{bmatrix}
s(\mathbf{z}_i^j, \mathbf{z}_1^*) &
s(\mathbf{z}_i^j, \mathbf{z}_2^*) & \dots& s(\mathbf{z}_i^j, \mathbf{z}_N^*)
\end{bmatrix}
\end{equation}
We use the softmax of $\hat{S}_i^j$ as the model's probability distribution on the label of $r_i^j$. The model is then trained to optimize the cross-entropy loss on this distribution against the gold label $\ell_i$.
% \dy{1. Do we need to explain why we want to get probabilities (i.e. why we use softmax) 2. is ``class representations" confusing here?}
% \xd{For 1. above, yes, some people might feel confused about the purpose of getting similarity at the first look; For 2., ``class representations'' look good to me.}\lh{it was a bit confusing to me .. i thought it was some kind of class embedding ...}

We experiment with three reduction functions, \textit{mean} (Eq.~\ref{eqa:mean}), \textit{max} (Eq.~\ref{eqa:max}), and \textit{min-max} (Eq.~\ref{eqa:min_max}):


\begin{equation}
\label{eqa:mean}
%%%%% NOTE: I use \Bigg because I hate the spacing of \left-\right -- Ice.
s(\mathbf{z}_i^j, \mathbf{z}_{i'}^*)
= \frac{1}{B}\sum_{j'=1}^B s(\mathbf{z}_i^j, \mathbf{z}_{i'}^{j'})
= s\Bigg(\mathbf{z}_i^j, \frac{1}{B} \sum\limits_{j'=1}^B \mathbf{z}_{i'}^{j'}\Bigg)
\end{equation}
\begin{equation}
\label{eqa:max}
s(\mathbf{z}_i^j, \mathbf{z}_{i'}^*) = \max_{\substack{1 \leq j' \leq B; \\ j' \neq j \text{ if } i = i'}} s(\mathbf{z}_i^j, \mathbf{z}_{i'}^{j'})
\end{equation}
\begin{equation}
\label{eqa:min_max}
s(\mathbf{z}_i^j, \mathbf{z}_{i'}^*) =
\begin{cases}
    \underset{1 \leq j' \leq B}{\min} s(\mathbf{z}_i^j, \mathbf{z}_{i'}^{j'}),  & \text{if } i = i'\\
    \underset{1 \leq j' \leq B}{\max} s(\mathbf{z}_i^j, \mathbf{z}_{i'}^{j'}),  & \text{otherwise}
\end{cases}
\end{equation}
%We abused the notation in Eq~\eqref{eqa:mean}: the sum refers to the sum of embedding vectors for spans~$\mathbf{z}_{i'}^{j'}$.
%\ice{This is quite a serious abuse since Eq 1 already hides the embeddings of $z_{i'}^{j'}$}
%\lh{I called the spans r and the embeddings z in the beginning of the section}
%\dy{Actually, all the z are contextual embeddings in all the equations. Since we defined z as the span in Setup, should we explain (maybe with a different notation here) at the beginning of this subsection?}

The \textit{mean} reduction averages embeddings of the spans with the same label and is equivalent to Prototypical Networks. Similar to hard negative sampling to increase margins among classes \cite{Schroffetal-2015-facenet, roth-etal-2020-revisiting, yang-etal-2019-improving}, \textit{max} takes the most similar span to the query (excluding the query itself) as the label representation, while \textit{min-max} takes the least similar span when considering spans with the same label as the query.
%We then train the encoder $E$ with cross-entropy loss to learn semantics related to class labels. \zy{Did you explain how you construct labels somewhere? It's straightforward but I think it's still worth one or two sentences.} 

% Our experiments show that \textit{max} (Eq.~\ref{eqa:max}) yields the best overall performance. 
% We will provide more analysis in Section~\ref{ana:intent} to study the the effectiveness of different reduction methods.
%\dy{revisit: we didn't compare with mean because we use proto instead}

%%%%% NOTE: MOVED TO FRONT OF 4.1
% In this paper, we use the public available pre-trained BERT-base uncase model \zy{Maybe add a link as footnote to the model?} as our encoder $E$ and dot product as our similarity function $s$. \footnote{We experimented with affine transformation as well as cosine similarity but did not see any performance gain. In addition, using the [CLS] token as the utterance representation achieves better results than averaging word embeddings in intent classification}
%but other encoders and similarity functions are also permissible
%%%%% END NOTE

\subsection{Inference}\label{sec:inference}
%We retrieve utterance level representation for intent classification.
%Different from previous works based on token-level retrieval \cite{wiseman-stratos-2019-label, hou-etal-2020-shot}, we retrieve examples at the span level for slot filling.
% \footnote{This can be seen as a special case with the span length equal to the utterance length.}. 
%\subsubsection{Slot filling}

%\dy{this is for inference time, right? should we move it to the next subsection?}

After training, we build a dense retrieval index where each entry $(r, \ell)$ is indexed by $\mathbf{z} = E(r)$.
The entries $(r, \ell)$ come from examples $(\mathbf{x}, \mathbf{y})$ in the \emph{support set} which,
depending on the setting,
could be just the target training data
or a mixture of source and target data.
For each query span $r'$ of the input utterance $\mathbf{x}$, we embed the span and compute the similarity scores against all index entries. 
% This process can be sped up by fast dot-product search algorithms~\cite{avq_2020}, though we found brute force computation to be sufficient.

\paragraph{Intent classification}
%In contrast to slot filling where we need to decode a sequence of spans with retrieved spans, there is only one span for intent classification with the length of the whole utterance.
%Intent classification can be seen as a straightforward special case of span labeling.
%Hence, predicting intent is straightforward. 
For intent classification, both index entries and query spans are restricted to the whole utterances. The entire process thus boils down to retrieving the most similar utterance based on the [CLS] token embedding. We simply output the intent label of the retrieved utterance.
%we simply use the [CLS] token embedding as the utterance representation and retrieve the most similar utterance in the support set where the retrieved label is the prediction. 

\paragraph{Slot filling}
\label{model_slot_decoding}
In contrast to BIO decoding for token-level similarity models~\cite{hou-etal-2020-shot}, decoding with span retrieval results poses unique challenges as gold span boundaries are not known a priori. Hence, 
% we decode the sequence of valid spans with beam search.
we use a modified beam search procedure with simple heuristics to compose the spans.
%Figure \ref{fig:illustration} illustrates the retrieving process.\xd{I think people might feel confused on where it illustrates the decoding process?} 
%\h{removed this line since this is too far from figure 1}
%For an utterance of length $n$, we first encode the utterance and compute span embeddings for all $n \times m$ spans

Specifically, for each of the $n \times m$ spans in an utterance of length $n$ (where the hyperparameter $m$ is the maximum span length), we retrieve the most similar span from the retrieval index.
% that is annotated with a slot name using the contextual span representation and
%using the similarity function introduced in Section~\ref{model:train}.
Then we normalize the similarity scores by L2-norm so that they are within the range $[0, 1]$. 
%\zy{How did you normalize the score?} 
% Since we do not explicitly learn span boundaries, all spans including ``book a table", ``black", ``black horse tavern" in Figure \ref{fig:illustration} will retrieve a span with a similarity score. However, invalid spans such as ``book a table" will have a low similarity score. Therefore, we filter all spans with a threshold to get potential spans. \zy{``Since we do not explicitly learn span boundaries'' is a bit confusing. Maybe directly state that ``Since we retrieve examples for each of the $n \times m$ spans''.}
Since we do not explicitly predict span boundaries, all $n \times m$ spans, including non-meaningful ones (e.g., \textit{``book a''}), will have a retrieved span. Such non-meaningful spans should be dissimilar to any labeled span in the retrieval index. We thus choose to filter the spans with a score threshold to get a smaller set of candidate spans. In addition, we adjust the threshold dynamically (by reducing the threshold for a few times) if no span is above the current threshold.
 
Once we get candidate spans with similarity scores, we use beam search to decode a set of spans with maximum average scores.\footnote{We use beam search for simplicity. Other search methods such as Viterbi algorithm \cite{forney-1973-viterbi} can also be used.}
%we convert the sequence tagging problem into a search problem with the goal of maximizing a pre-defined sequence metric.
% Previous token-level retrieval models leverages Viterbi algorithm \cite{forney-1973-viterbi} for decoding. 
% However, Viterbi decodes a sequence that maximizes the overall similarity scores by incorporating all possible spans which would assign a span to each token even if the token is not part of any valid spans. In addition, because potential spans can overlap with each other, the number of states, i.e., potential spans, can be large and expensive to compute. Therefore, 
We go through the list of candidate spans in the descending order of their similarity scores. For each candidate span, we expand beam states if the span does not overlap with the existing spans in the beam.
%span to the output and exclude any states that contain overlapping spans. 
The search beams are pruned based on the average similarity score of the spans included so far. Lastly, we add spans in the filtered set which do not overlap with the final beam.

Beam search can avoid suboptimal decisions that a greedy algorithm would make.
% We start by sorting all the candidate spans by similarity scores. One simple option is to choose the span with the highest score and the next non-overlapping span until no span is left.
For instance, if we greedily process the example in Figure~\ref{fig:illustration},
%\textit{``tavern''} will be decoded first, followed by \textit{``black''}.
% \dy{should we include the target output in the figure (e.g. highlight the query spans) or in the caption?}
%The sequence hereby decodes
\textit{``black''} and \textit{``tavern''} would become two independent spans, even though their average similarity score is lower than the correct span \textit{``black horse tavern''}.
%Thus, we use beam search to predict the span sequence that maximizes the average similarity score. 
%
% Finally, although beam search optimizes a sequence of hypotheses,
% our decoding procedure
Nevertheless, beam search
is prone to mixing up span boundaries and occasionally predicts consecutive partial spans such as \textit{``black horse''} and \textit{``tavern''} as individual slots.
%Compared to other sequence labeling tasks such as part-of-speech tagging where consecutive individual spans sharing the same type is prevalent, we found that
Since consecutive spans of the \emph{same} slot label are rare in slot filling datasets, we merge the two spans if their retrieval scores are within a certain range:
\begin{equation}
\label{eqa:merge}
\small
    r_{i:j}, r_{j:k} = 
    \begin{cases}
        r_{i:k} & \text{if } |s(\mathbf{z}_{i:j}, \mathbf{z}') - s(\mathbf{z}_{j:k}, \mathbf{z}'')| < \lambda\\
        r_{i:j}, r_{j:k} & \text{otherwise} \nonumber
    \end{cases}
\end{equation}
where $r_{i:j}$ and $r_{j:k}$ are two consecutive potential spans sharing the same label, and $\mathbf{z}'$ and $\mathbf{z}''$ are the embeddings of their retrieved spans, respectively ($r_{i:k}$ indicates merging the two spans into one span; $\lambda$ is the merge threshold where $\lambda = 1$ means always merge and $\lambda = 0$ means never merge).
 

==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/related_work.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Few-shot metric learning}
% Unlike optimization-based methods that adapt model parameters for few-shot learning such as meta-learning \cite{finn-etal-2017-meta, mishra-etal-2018-meta},\ice{Meta-learning seems a bit out-of-place. The only relation to metric learning seems to be that it's used in few-shot tasks.}
Metric learning methods target at learning representations through distance functions. \citet{koch-etal-2015-siamese} proposed Siamese Networks which differentiated input examples with contrastive and triplet loss functions~\cite{Schroffetal-2015-facenet} on positive and negative pairs. 
While they are more data efficient for new classes than linear classifiers, Siamese Networks are hard to train due to weak pairs sampled from training batch \cite{gillick-etal-2019-learning}.
% \ice{Is this true? I thought they sample positive + negative pairs and not doing all $O(n^2)$ pairs.} 
In comparison, Prototypical Networks \cite{snell-etal-2017-prototypical} proposed to compute class representations by averaging embeddings of support examples for each class. 
These methods
% show better performance over Siamese Networks and
have been mostly explored in computer vision and text classification~\cite{geng-etal-2019-induction, yu-etal-2018-diverse}, and 
% These prototype representation-based methods also 
consistently outperform Siamese Networks and retrieval-based methods such as \textit{k}-nearest-neighbors,  especially when there are more classes and fewer annotated examples \cite{meta_dataset, sun-etal-2019-hierarchical}.
However, newly added examples which are outliers may change the prototypical representations dramatically that can harm all predictions on the class.
% However, in domain transfer scenarios, newly added examples may not update the prototype representation so that a similar query to the support example may not be classified correctly.\ice{I don't understand this sentence.} \dy{re: two cons of prototypical: 1. outliers can change the prototypical representation dramatically, thus harming all predictions on this class 2. new added examples may not update prototypical representation enough so that queries cannot be classified correctly (such as hot-fix)} 
In addition, these methods do not perform well when there are more annotated data available per class \cite{meta_dataset}.

Recently, \citet{wang-etal-2019-simpleshot} showed that a simple nearest neighbor model with  feature transformations can achieve competitive results with the state-of-the-art methods on image classification. Inspired by their work, we train our retrieval-based model with a novel batch softmax objective. 
%We show that our retrieval-based method achieve better performances than other strong metric learning methods, even though previous \textit{k}-NN methods often under-perform when the support set is small. 


\paragraph{Metric learning in language understanding}
Utilizing relevant examples to boost model performance has been applied to language modeling \cite{khandelwal-etal-2020-generalization}, question answering \cite{guu2020realm, lewis2020retrievalaugmented}, machine translation \cite{zhang-etal-2018-guiding}, and text generation \cite{peng-etal-2019-text}. 
Recently, metric learning has been applied to intent classification \cite{sun-etal-2019-hierarchical, krone-etal-2020-learning}. \citet{ren-etal-2020-intention} trained Siamese Networks before learning a linear layer for intent classification and showed competitive results with traditional methods in the full-data setting. 
Similar ideas are also extended to sequence labeling tasks such as named entity recognition (NER, \citealp{wiseman-stratos-2019-label, fritzler-etal-2018-fewshot}) by maximizing the similarity scores between contextual tokens representations sharing the same label.
\citet{krone-etal-2020-learning} utilized Prototypical Networks to learn intent and slot name prototype representations and classified each token to its closest prototype. They showed better results than meta-learning, another prevalent few-shot learning method \cite{finn-etal-2017-meta, mishra-etal-2018-meta}.
% on intent classification and slot filling tasks.  
In order to consider label dependencies that are essential in slot tagging tasks \cite{huang-etal-2015-bidirectional}, %but ignored in previous work, 
\citet{hou-etal-2020-shot} proposed a collapsed dependency transfer (CDT) mechanism by simulating transition scores for the target domain from transition probabilities among BIO labels in the source domain, outperforming previous methods on slot filling by a large margin. 
\citet{yang-katiyar-2020-simple} further explored the transition probability by evenly distributing the collapsed transition scores to the target domain to maintain a valid distribution. 
However, this simulation is noisy and the difference between the source and target domains can result in biased transition probabilities.

The most similar approach to ours is a concurrent work from~\citet{ziyadi-etal-2020-example}, which learns span boundaries and sentence similarities before retrieving the most similar span, inspired by question-answering models. 
% Even though this approach focuses on learning span boundaries and
Even though this approach predicts spans before retrieving on the span level and thus bypasses the problem of transition probability in previous research, it only achieves unsatisfactory results. 
Different from these researches, we propose to learn span representations using a batch softmax objective without having to explicitly learn span boundaries. Our method achieves more accurate slot and intent prediction than previous methods in the few-shot setting.

==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/setup.tex <==
\section{Setup}\label{sec:setup}

We consider two tasks where the input is an utterance $\mathbf{x}$ with tokens $x_1, \dots, x_n$ and the output is some structure $\mathbf{y}$.
For the \emph{slot filling} task, the output $\mathbf{y}$ is a set of non-overlapping labeled spans $\{(r_i, \ell_i)\}_{i=1}^m$ where $r_i$ is a span of $\mathbf{x}$ (e.g., \emph{``7 pm''}) and $\ell_i$ is a slot name (e.g., \texttt{time}). For the \emph{intent classification} task, the output $\mathbf{y}$ is simply an intent label $\ell$ for the whole utterance $\mathbf{x}$. For notational consistency, we view intent classification as predicting a labeled span $(r, \ell)$ where $r = \mathbf{x}_{1:n}$.

In the few-shot setup,
examples $(\mathbf{x}, \mathbf{y})$ are divided into \emph{source} and \emph{target} domains.
Examples in the target domain may contain some labels $\ell$ that are unseen in the source domain.
The model will be given ample training data from the source domain, but only a few training examples from the target domain. For instance, the model receives only $K = 5$ examples for each unseen label.
The model can be evaluated on test data from both domains.

==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/tables/clinc_comp_results.tex <==
\begin{table}[t]
\small
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccc}
\toprule
% & \multicolumn{2}{c}{5-shot} & \multicolumn{2}{c}{2-shot} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
& tgt   & src  & avg  \\ 
\midrule
\texttt{BERT fine-tune} & - & - & - \\
\texttt{Proto} & +12.89 & -0.51 & +5.18 \\
\texttt{Retriever} & \textbf{+14.60} & \textbf{-0.14} & \textbf{+6.11}  \\
\texttt{Retriever min-max} & +10.79 & -0.20 & +4.47 \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{\label{clinc_comp_results} Improvement (\%) over \texttt{BERT fine-tune} on target (tgt), source (src), and average (avg), after fine-tuning on the 5-shot support sets. Numbers are averaged over different ($n_c, n_i$) data samples.}
% \vspace{-1em}
\end{table}


% \begin{table}[t]
% \small
% \begin{center}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lcccc}
% \toprule
% & \multicolumn{2}{c}{5-shot} & \multicolumn{2}{c}{2-shot} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
% & tgt   & src  & tgt & src  \\ 
% \midrule
% \texttt{BERT} fine-tune & - & - & - & - \\
% \texttt{Proto} & +12.89 &	-0.51 & \textbf{+16.39} & \textbf{-0.27} \\
% \texttt{Retriever} & \textbf{+14.60} & \textbf{-0.14} & +15.78 & -1.52 \\
% \texttt{Retriever min-max} & +10.79 & -0.20 & +12.72 & -0.59  \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \caption{\label{clinc_comp_results} Improvement (\%) over \texttt{BERT} fine-tune on target (tgt) and source (src) domains, after fine-tuning on the target domains, with 5-shot and 2-shot support sets. 
% Negative numbers represent worse performance. }
% % \vspace{-1em}
% \end{table}


% \begin{table}[h]
% \small
% \begin{center}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lcccccc}
% \toprule
% & \multicolumn{3}{c}{5-shot} & \multicolumn{3}{c}{2-shot} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7}
% & tgt   & src  & avg. & tgt & src  & avg.  \\ 
% \midrule
% \texttt{BERT} fine-tune & - & - & - & - & - & - \\
% \texttt{Proto} & +12.89 &	-0.51 & +5.18 & \textbf{+16.39} & \textbf{-0.27} & \textbf{+6.33}\\
% \texttt{Retriever} & \textbf{+14.60} & \textbf{-0.14} & \textbf{+6.11} & +15.78 & -1.52 & +5.33 \\
% \texttt{Retriever min-max} & +10.79 & -0.20 & +4.47 & +12.72 & -0.59 & +4.68 \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \caption{\label{clinc_comp_results} Improvement (\%) over \texttt{BERT} fine-tune on target, source, and all domains (avg), after fine-tuning on the target domains, with 5-shot and 2-shot support sets. 
% Negative numbers represent worse performance. }
% \vspace{-1em}
% \end{table}


==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/tables/clinc_results.tex <==
\begin{table*}[t]
\footnotesize
\begin{center}
%\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccc|ccc|c}
\toprule
& \multicolumn{3}{c|}{support\_set=all} & \multicolumn{3}{c|}{support\_set=balance} & support\_set=tgt \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-8}
& tgt   & src  & avg   & tgt & src & avg   & tgt  \\ 
\midrule
\multicolumn{4}{l}{\textit{Initial BERT }}     \\
\midrule
$\texttt{Proto}^{\texttt{frz}}$ & 14.07 & 25.02 & 21.37 & - & - & - & -\\
$\texttt{Retriever}^{\texttt{frz}}$ & 8.24 & 54.76 & 39.25 & 22.09 & 25.29 & 24.22 & 37.93\\
\midrule
\multicolumn{4}{l}{\textit{Pre-train on src domain }} \\  
\midrule
\texttt{BERT fine-tune} & - & 96.51 & - & - & - & - & -\\ 
\texttt{Proto} & 75.02 & 95.73 & 88.83 & - & - & - & -\\ 
\texttt{Retriever} & 62.69 & \textbf{97.08} & 85.62 & 75.93 & 95.44 & 88.94 & 88.53\\
\texttt{Retriever  min-max} & 66.00 & 96.64 & 86.43 & 71.82 & 95.14 & 87.37 & 86.38\\
\midrule
\multicolumn{4}{l}{\textit{Fine-tune on tgt domain }} \\
\midrule 
\texttt{BERT fine-tune} & 78.89 & 43.91 & 55.57 & - & - & - & -\\
\texttt{Proto} & 80.44 & 95.57 & 90.53 & - & - & - & 90.35\\
\texttt{Retriever} & 66.76 & 96.95 & 86.89 & 79.20 & 95.50 & 90.07 & \textbf{91.16}\\
\texttt{Retriever  min-max} & 67.64 & 96.84 & 87.11 & 77.60 & 95.35 & 89.43 & 89.56\\
\midrule 
\multicolumn{4}{l}{\textit{Fine-tune on tgt domain with src data}} \\ 
\midrule 
% BERT FT & 64.69 & 96.14 & 80.42 & - & - & - & -\\ 
\texttt{BERT  fine-tune} & 72.00 & 95.18 & 87.45 & - & - & - & -\\ 
\texttt{Proto} & 83.33 & 94.82 & 90.99 & - & - & - & 90.22\\
\texttt{Retriever} & 69.51 & 97.04 & 87.86 & \textbf{84.95} & 95.41 & \textbf{91.92} & 90.78\\
\texttt{Retriever  min-max} & 71.35 & 96.96 & 88.42 & 81.00 & 94.55 & 90.03 & 89.82\\

\bottomrule
\end{tabular}
%}
\end{center}
\caption{\label{clinc_results} Intent accuracy on CLINC for $n_c=10, n_i=10$ with 5-shots. Our retrieval-based method outperform BERT fine-tune and Prototypical Networks in both target and source domains. We report results for our method when the support set consists of all examples in the source and target domains (all), when the support set consists of balanced few-shot number of examples for intents in both source and target domains (balance), and when the support set consists of examples of the target domain only (tgt) which serves as an upper-bound.}
\vspace{-1em}
\end{table*}

==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/tables/snips_beam.tex <==
\begin{table}[t]
\footnotesize
\begin{center}
\small
%\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{ccc}
\toprule
beam size  & merge threshold & avg. F1  \\ 
\midrule
1 & 0.99 & 70.10 \\
5 & 0.99 & 71.47 \\
10 & 0.99 & 71.72 \\
10 & 0 & 70.43 \\
10 & 1 & 72.10 \\
\bottomrule
\end{tabular}
%}
\end{center}
\caption{\label{snips_beam} Ablation study on beam size and merge condition.  Merge threshold of 0 means never merge and 1 means always merge. Using larger beam and merging consecutive spans improve F1 scores.
% \lh{merge with the merge threshold one as one ablation table?}
}
\vspace{-1em}
\end{table}

==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/tables/snips_merge.tex <==
\begin{table}[t]
\small
\begin{center}
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{cc}
\toprule
merge threshold   & avg. F1  \\ 
\midrule
0 & 70.43 \\
1 & 72.10 \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{\label{snips_merge} Ablation study on merge condition, where $0$ means never merge and $1$ means always merge. Merging consecutive spans improve F1 scores.}
\end{table}

==> Few-shot Slot Filling and Intent Classification with Retrieved Examples/tables/snips_results.tex <==
\begin{table*}[t]
\footnotesize
\begin{center}
%\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccccc|c}
\toprule
& GW   & PM    & ATP    & RB    & FSE    & BR    & SCW   & Average F1  \\ 
\midrule
\multicolumn{1}{l}{\textit{Classification-based}}     \\
\midrule
\texttt{BERT Tagging}  & 59.41 & 42.00 & 46.07 & 20.74 & 28.20 & 67.75 & 58.61 & 46.11 \\
\midrule
\multicolumn{1}{l}{\textit{Token-level}}     \\
\midrule
$\texttt{SimilarToken}^{\texttt{frz}}$ & 53.46 & 54.13 & 42.81 & 75.54 & 57.10 & 55.30 & 32.38 & 52.96  \\
\texttt{MatchingToken} & 36.67 & 33.67 & 52.60 & 69.09 & 38.42 & 33.28 & 72.10 & 47.98 \\
\texttt{ProtoToken}  & 67.82 & 55.99 & 46.02 & 72.17 & \textbf{73.59} & 60.18 & \textbf{66.89} & 63.24 \\
\texttt{L-TapNet+CDT+Proto} & - & - & - & - & - & - & - & 67.27\\ 
$\texttt{L-Proto+CDT}^\texttt{pw}$* & 74.68 & 56.73 & 52.20 & 78.79 & 80.61 & 69.59 & 67.46 & 68.58\\
$\texttt{L-TapNet+CDT+Proto}^\texttt{pw}$* & 71.64 & 67.16 & 75.88 & 84.38 & 82.58 & 70.05 & 73.41 & 75.01\\ 

\midrule
\multicolumn{1}{l}{\textit{Span-level (ours)}}     \\
\midrule
$\texttt{Proto}^{\texttt{frz}}$ & 39.47 & 38.35 & 47.68 & 69.36 & 38.60 & 42.39 & 19.90 & 42.25 \\
\texttt{Proto} & 64.47 & 53.97 & 54.64 & 73.37 & 42.89 & 62.48 & 27.76 & 54.23 \\
$\texttt{Retriever}^{\texttt{frz}}$ & 63.39 & 46.01 & 51.11 & 79.65 & 62.42 & 62.13 & 33.85 & 56.94 \\
\texttt{Retriever} & \textbf{82.95} & \textbf{61.74} & \textbf{71.75} & \textbf{81.65} & 73.10 & \textbf{79.54} & 51.35 & \textbf{71.72} \\
% \midrule
% \multicolumn{1}{l}{\textit{Model with pair-wise embeddings}}     \\

\bottomrule
\end{tabular}
%}
\end{center}
\caption{\label{tab:snips_results} Results on SNIPS test data with 5-shot support sets. Our span-based retrieval model outperforms previous classification-based and token-level retrieval models even without label semantics. Classification-based and token-level results are reported in \citet{hou-etal-2020-shot}. *Pair-wise embeddings (marked with $^{\texttt{pw}}$) are expensive at inference time, so we do not compare our method with these directly. 
% \dy{if we present the results this way, how should we highlight(bold) the numbers?}
}
\vspace{-1em}
\end{table*}

==> introduction_old.tex <==
\section{Introduction}
\lh{The intro feels a lot better length-wise. I think we probably need to work more on the motivation part.}

Few-shot learning scenarios are prevalent and are challenging to data-intensive supervised learning methods. For instance, there are constant expansions to new domains and labels to support more tasks but there may only be few annotated data points for these new labels. Motivated by this, we focus on cross-domain adaptation by training on the source domains with larger amounts of data, and then apply the trained model to the target domain with only few annotated examples on slot filling and intent classification tasks.


% Structured prediction such as slot filling and text classification such as intent classification are essential natural language understanding tasks.
% % in task-oriented dialog systems. 
% For example, in task-oriented dialog systems, given a user utterance ``I'd like to book a table at black horse tavern at 7 pm'', the slot filling task is to find task-related slot values such as ``\texttt{7 pm}'' and the corresponding slot names such as ``\texttt{time range}'' in a structured prediction paradigm. The intent classification task is to classify the utterance to the ``\texttt{restaurant booking}'' class. 
% %Similarly, the intent classification task is to find the user intent for the whole utterance. 
% In virtual assistants such as Alexa and Google Assistant, few-shot learning scenarios are prevalent and are challenging to data-intensive supervised learning methods.
% For instance, there are constant expansions to new domains and labels during deployment to support more tasks but there may only be few annotated data points for these new labels. 
% %In addition, changing of annotation schemas such as using more fine-grained annotation can also be considered as few-shot setting. 
% Motivated by this, we focus on cross-domain adaptation by training on the source domains with larger amounts of data, and then apply the trained model to the target domain with only few annotated examples.

% Traditionally, researchers leverage linear classification models on top of neural encoders to predict BIO labels with linear conditional random fields (CRFs, \citealp{lafferty-etal-2001-conditional}) for slot filling, and to predict intent classes with a linear layer for intent classification \cite{mesnil-etal-2014-using, lample-etal-2016-neural, goo-etal-2018-slot}. Even though large language model pre-training boosts the performance on both tasks \cite{peters-etal-2018-deep, devlin-etal-2019-bert}, these models are often data intensive and do not work well for few-shot settings due to overfitting with inductive bias \cite{snell-etal-2017-prototypical, meta_dataset} and catastrophic forgetting problems on the source domain \cite{wu-etal-2019-transferable}.

Traditionally, researchers leverage linear classification models for slot filling and intent classification \cite{mesnil-etal-2014-using, lample-etal-2016-neural, goo-etal-2018-slot} and more recently, with pre-trained language models \cite{peters-etal-2018-deep, devlin-etal-2019-bert}. However, these models are often data intensive due to the bottleneck of learning linear layers for labels. Thus they suffer from overfitting with inductive bias  in few-shot settings. In addition, they are prone to catastrophic forgetting on the source domain \cite{wu-etal-2019-transferable}.

% An alternative direction is metric learning \cite{vinyals-etal-2016-matching, snell-etal-2017-prototypical} to learn embedding representations which has shown superior performance for few-shot settings in both vision and language tasks.
% Similar to GPT-3 \cite{brown-etal-2020-langauge}, these methods do not require fine-tuning the whole model on new domains which have limited annotated examples, thus are less susceptible to overfitting and catastrophic forgetting problems. More importantly, these methods decouples learned models from the semantics by only associating semantics with the retrieval index.
%, and thus are robust to schema changes and simplify point-fixing.
% Recently, metric learning methods such as Prototypical Networks \cite{snell-etal-2017-prototypical} have been applied to slot filling and intent classification tasks \cite{wiseman-stratos-2019-label, hou-etal-2020-shot, sun-etal-2019-hierarchical} and performance gains have been observed. However, they focus on token-level similarity learning and either ignore or simulate a noisy bi-gram label dependency to decode a sequence of label predictions. In addition, performance on the source domain where we have more training examples is critical, but \citet{meta_dataset} showed that these methods perform poorly in this setting compared to fine-tuning.

An alternative approach is metric learning \cite{weinberger-etal-2006-distance, vinyals-etal-2016-matching, snell-etal-2017-prototypical}. These models are usually based on similarity models rather than task-specific classifiers, allowing decoupling the learned models from the semantics by only associating semantics with the retrieval index. Since methods such as nearest neighbor retrieval map queries to the neighborhood around each support example, they are less susceptible to catastrophic forgetting and data imbalance between the source and target domains. 
These benefits make it appealing to apply to few-shot settings.
Recently, metric learning methods such as Prototypical Networks \cite{snell-etal-2017-prototypical} have been applied to slot filling and intent classification tasks \cite{wiseman-stratos-2019-label, hou-etal-2020-shot, sun-etal-2019-hierarchical}. 
However, they focus on token-level similarity learning for slot tagging and either ignore or simulate a noisy bi-gram label transition probabilities to decode a sequence of tags. 


%\lh{maybe emphasis that in previous paragraphs that most of the few-shot learning literature focus on intent classification and doesn't work well with structured prediction tasks}
In this paper, we propose to learn span-level similarity retrieval models and decode the retrieved spans to a valid structure. 
In addition to the benefits of metric learning and other non-parametric models such as GPT-3 \cite{brown-etal-2020-langauge} in the few-shot setting,
retrieval-based methods are less sensitive to outliers in prototype representations and can also perform well in large-shot settings compared to methods such as Prototypical Networks.
% we fine-tune BERT \cite{devlin-etal-2019-bert} using batch softmax to learn similar representations to spans sharing the same label with hard examples on the source domain.
\dy{does "two-tower model" indicate dual-encoder? Note that we are very different from dual encoder models}
During training, we fine-tune a two-tower model with BERT \cite{devlin-etal-2019-bert} encoders to enforce high similarity between span embeddings sharing the same label.
We introduce a novel batch softmax loss and empirically show that it performs better than other methods.
At inference time, we retrieve the most similar span from the few-shot in-domain examples to each potential span and decode a set of spans that has the maximum average similarity score.
%as the sequence prediction.
We then expand the span-level retrieval to utterance-level retrieval for intent classification. 
We show that our proposed method is effective by
evaluating it on SNIPS \cite{coucke-etal-2018-snips} for slot filling and CLINC \cite{larson-etal-2019-evaluation} for the intent classification task independently.
\dy{I focused on highlighting the benefits/motivation of using retrieval vs. prototypcal, i.e. less sensitive to outliers; work well for large-shots. However, I think the benefits of 1. interpretable 2. deterministic and hot-fix, (3. fast decoding) should also be mentioned here.}

% Moreover, our retrieval-based method is interpretable, and the prediction is deterministic once the examples are added, compared to methods such as Prototypical Networks.
% Moreover, span-level retrieval can lift the requirement of sequential dependencies and thus speed up the decoding procedure, similar to non-autoregressive slot tagging.
% We show that our proposed method is effective by
% evaluating it on SNIPS \cite{coucke-etal-2018-snips} for slot filling and CLINC \cite{larson-etal-2019-evaluation} for the intent classification task independently.

==> tables/snips_merge.tex <==
\begin{table}[t]
\small
\begin{center}
\resizebox{0.6\columnwidth}{!}{
\begin{tabular}{cc}
\toprule
merge threshold   & avg. F1  \\ 
\midrule
0 & 70.43 \\
1 & 72.10 \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{\label{snips_merge} Ablation study on merge condition, where $0$ means never merge and $1$ means always merge. Merging consecutive spans improve F1 scores.}
\end{table}
